Exploring Transformers for Open-world Instance Segmentation

Open-world instance segmentation is a rising task, which aims to segment all objects in the image by learning from a limited number of base-category objects. This task is challenging, as the number of unseen categories could be hundreds of times larger than that of seen categories. Recently, the DETR-like models have been extensively studied in the closed world while stay unexplored in the open world. In this paper, we utilize the Transformer for open-world instance segmentation and present SWORD. Firstly, we introduce to attach the stop-gradient operation before classification head and further add IoU heads for discovering novel objects. We demonstrate that a simple stop-gradient operation not only prevents the novel objects from being suppressed as background, but also allows the network to enjoy the merit of heuristic label assignment. Secondly, we propose a novel contrastive learning framework to enlarge the representations between objects and background. Specifically, we maintain a universal object queue to obtain the object center, and dynamically select positive and negative samples from the object queries for contrastive learning. While the previous works only focus on pursuing average recall and neglect average precision, we show the prominence of SWORD by giving consideration to both criteria. Our models achieve state-of-the-art performance in various open-world cross-category and cross-dataset generalizations. Particularly, in VOC to non-VOC setup, our method sets new state-of-the-art results of 40.0% on ARb100 and 34.9% on ARm100. For COCO to UVO generalization, SWORD significantly outperforms the previous best open-world model by 5.9% on APm and 8.1% on ARm100.

==> tables/ab_topk.tex <==
\begin{tabular}{c| ccc| ccc}
\Xhline{1.0pt}

\multirow{2}{*}{top-$k$} & \multicolumn{3}{c|}{Novel}  & \multicolumn{3}{c}{All} \\
%  & \multicolumn{3}{c|}{Box} & \multicolumn{3}{c|}{Mask} & 
%   \multicolumn{3}{c|}{Box} & \multicolumn{3}{c|}{Mask} \\
\cline{2-7} 
 & AP$^{\rm b}$ & AR$_{10}^{\rm b}$ & AR$_{100}^{\rm b}$
 & AP$^{\rm b}$ & AR$_{10}^{\rm b}$ & AR$_{100}^{\rm b}$ \\
\Xhline{1.0pt}

0 & 14.2 & 20.0 & 45.8 & 29.1 & 35.0 & 60.7 \\
1 & 15.4 & 21.5 & 47.5 & 28.8 & 35.6 & 61.3 \\
3 & 16.7 & 22.6 & 49.8 & 28.4 & 35.2 & 62.5 \\
5 & 16.7 & 22.4 & 49.8 & 26.8 & 34.1 & 62.4 \\
10 & 15.3 & 21.3 & 51.1 & 22.8 & 31.1 & 61.7 \\
            

\Xhline{1.0pt}
\end{tabular}

==> tables/strong_aug.tex <==
\begin{tabular}{c|c|c|l}
\Xhline{1.0pt}
\multicolumn{4}{c}{\textbf{Strong Augmentation}}\\ 
\hline
\hline
Augmentation & Probability & Parameters& \multicolumn{1}{c}{Descriptions}\\
\midrule

Color Jittering & 0.8                     & \begin{tabular}[c]{@{}c@{}}(brightness, contrast, saturation, hue)\\ = (0.4, 0.4, 0.4, 0.1)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Brightness factor is chosen uniformly from {[}0.6, 1.4{]},\\ contrast factor is chosen uniformly from {[}0.6, 1.4{]},\\ saturation factor is chosen uniformly from {[}0.6, 1.4{]},\\ and hue value is chosen uniformly from {[}-0.1, 0.1{]}.\end{tabular} \\ 

\midrule
Grayscale       & 0.2                     & None                                                                                                       & \multicolumn{1}{c}{None}                                                                                                                                                                                                                                                                                    \\  \midrule
GaussianBlur    & 0.5                     & (sigma\_x, sigma\_y) = (0.1, 2.0)                                                                        & Gaussian filter with $\sigma_x=0.1$ and $\sigma_y=2.0$ is applied.                                                                                                                                                                                                                   \\ \midrule
CutoutPattern1  & 0.7                     & scale=(0.05, 0.2),  ratio=(0.3, 3.3)                                                                     & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern2  & 0.5                     & scale=(0.02, 0.2), ratio=(0.1, 6)                                                                        & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels.\end{tabular}                                                                                                                                             \\ \midrule
CutoutPattern3  & 0.3                     & scale=(0.02, 0.2), ratio=(0.05, 8)                                                                       & \begin{tabular}[c]{@{}l@{}}Randomly selects a rectangle region in an image\\  and erases its pixels.\end{tabular}
\\
\Xhline{1.0pt}
\end{tabular}

==> tables/voc2uvo.tex <==
\begin{tabular}{l| ccc|ccc| ccc|ccc}
\Xhline{1.0pt}

\multirow{2}{*}{Method} & \multicolumn{6}{c|}{Novel}  & \multicolumn{6}{c}{All} \\
%  & \multicolumn{3}{c|}{Box} & \multicolumn{3}{c|}{Mask} & 
%   \multicolumn{3}{c|}{Box} & \multicolumn{3}{c|}{Mask} \\
\cline{2-13} 
 & AP$^{\rm b}$ & AR$_{10}^{\rm b}$ & AR$_{100}^{\rm b}$
 & AP$^{\rm m}$ & AR$_{10}^{\rm m}$ & AR$_{100}^{\rm m}$ 
 & AP$^{\rm b}$ & AR$_{10}^{\rm b}$ & AR$_{100}^{\rm b}$ 
 & AP$^{\rm m}$ & AR$_{10}^{\rm m}$ & AR$_{100}^{\rm m}$ \\
\Xhline{1.0pt}

LDET      & 9.3 & 16.0 & 31.9 & 4.9 & 12.3 & 25.2 & 22.7 & 28.1 & 43.3 & 18.7 & 23.9 & 36.0 \\
Deformable-DETR 
          & 7.2 & 13.5 & 33.5 & 3.4 & 9.5 & 25.3 & 23.4 & 29.4 & 49.8 & 19.1 & 24.0 & 39.4 \\
\hline

\modelname{} 
          & 11.2 & 16.8 & 43.1 & 6.1 & 13.3 & 34.9 & \textbf{24.9} & 30.6 & 55.3 & 19.6 & 25.3 & 45.2 \\
\modelname{}$^{*}$ 
          & \textbf{11.8} & \textbf{18.4} & \textbf{45.6} & \textbf{8.4} & \textbf{16.8} & \textbf{38.1} & 23.4 & \textbf{31.1} & \textbf{59.2} & \textbf{21.0} & \textbf{28.4} & \textbf{49.5} \\
            

\Xhline{1.0pt}
\end{tabular}
